ScopeBind: Attributing Edited Images to Registered Watermarked Releases

Attributing an edited image to a registered watermarked release faces a central tension: visual retrieval can match an edited image to its archived original even when it never descended from a watermarked release, whereas generative reconstruction often preserves scene content while erasing readable watermark codes. We present ScopeBind, a registered-release attribution framework that recovers exact release identifiers without a candidate claim at inference. ScopeBind combines global and local watermark hypotheses with a conditional original-gallery proposal, then verifies each candidate via a release-specific orthogonal latent decomposition derived from the registered original-release pair. Projecting the query displacement onto the issuance direction measures alignment with the watermarked release, while the orthogonal remainder retains content-consistency evidence that cancels out of endpoint distances. Using the same representation, a constrained manifold-aligned fusion rule strengthens watermark survivability before registration without retraining the codecs. Across natural and generated domains, ScopeBind reaches up to 97.50% and 89.38% exact attribution under strong generative reconstruction, outperforming the strongest public baseline by over 34 percentage points on COCO while keeping transfer and unmarked false acceptances near zero. Cross-editor tests on Stable Diffusion XL and InstructPix2Pix, writer-transfer studies, and gallery scaling to 10,000 originals confirm its robustness and scalability.

==> experiment-placement.tex <==
\usepackage{cuted,multicol}
\makeatletter
\newcommand{\ScopeLegacyColumns}[2]{%
  \par\noindent\begin{minipage}[t]{\dimexpr(\linewidth-\columnsep)/2\relax}%
  \vspace{0pt}#1\end{minipage}\hfill
  \begin{minipage}[t]{\dimexpr(\linewidth-\columnsep)/2\relax}%
  \vspace{0pt}#2\end{minipage}\par}
\newcommand{\SBPanel}[1]{\par\vspace{2pt}\noindent\begin{minipage}{\linewidth}\def\@captype{figure}#1\end{minipage}\par\vspace{3pt}}
\newcommand{\SBTablePanel}[1]{\par\vspace{3pt}\noindent\begin{minipage}{\linewidth}\def\@captype{table}#1\end{minipage}\par\vspace{6pt}}
\newcommand{\ScopeInlineTable}[1]{%
  \SBTablePanel{\RenewDocumentEnvironment{table*}{O{}}{}{}\input{tables/#1}}}
\makeatother

\newcommand{\ScopeColumns}[2]{%
  \par\begingroup\setlength{\multicolsep}{4pt}%
  \begin{multicols}{2}#1\space#2\end{multicols}\endgroup\par}
\BeforeBeginEnvironment{IEEEbiography}{\par\noindent\begin{minipage}[t]{\linewidth}}
\AfterEndEnvironment{IEEEbiography}{\end{minipage}\par\vspace{12pt}}
\makeatletter
\newcommand{\SBNeedspace}[1]{\@IEEEtranneedspace{#1}{\relax}}
\makeatother

